C3DAG: Controlled 3D Animal Generation using 3D pose guidance

Recent advancements in text-to-3D generation have demonstrated the ability to generate high quality 3D assets. However while generating animals these methods underperform, often portraying inaccurate anatomy and geometry. Towards ameliorating this defect, we present C3DAG, a novel pose-Controlled text-to-3D Animal Generation framework which generates a high quality 3D animal consistent with a given pose. We also introduce an automatic 3D shape creator tool, that allows dynamic pose generation and modification via a web-based tool, and that generates a 3D balloon animal using simple geometries. A NeRF is then initialized using this 3D shape using depth-controlled SDS. In the next stage, the pre-trained NeRF is fine-tuned using quadruped-pose-controlled SDS. The pipeline that we have developed not only produces geometrically and anatomically consistent results, but also renders highly controlled 3D animals, unlike prior methods which do not allow fine-grained pose control.

==> sec/4_experiment.tex <==
\section{Experiment}
\label{sec:experiment}

todo:  add perpneg

\subsection{Training protocol for ControlNet}
\subsubsection{Training dataset creation}

\subsection{End-to-End avatar generation}

\subsection{Evaluation of generated avatars}





% \subsubsection{Quantitative evaluation}

\subsubsection{Qualitative evaluation}
OOD - extinct creatures: tasmanian tiger, cartoon characters?



\subsection{Ablation Studies}

\subsection{Efficiency}

\subsection{Applications and Extensibility}


Animals:
Tiger
Bird
elephant

Compare MVDream:
komodo dragon
chameleon
alligator
axolotl
NO POSE CONTROL

OOD:
Pink Panther
other pop culture
extinct
3 headed monster
godzilla

Comparison Text-to-3D:
stable dreamfusion perpneg
HiFA


Comparison animal gen:
SMAL
LASSIE
MagicPony
Learning the 3D Fauna of the Web

Comparison starting from SMAL:
with controlnet perpneg
with controlnet
w/o controlnet perpneg
w/o controlnet 


Ablation:
Start with nothing
Start with SMAL
Start with balloons 


with and without dmtet?



Human Study


